VST-A: A Foundationally Sound Annotation Verifier

Program verifiers for imperative languages such as C may be annotation-based, in which assertions and invariants are put into source files and then checked, or tactic-based, where proof scripts separate from programs are interactively developed in a proof assistant such as Coq. Annotation verifiers have been more automated and convenient, but some interactive verifiers have richer assertion languages and formal proofs of soundness. We present VST-A, an annotation verifier that uses the rich assertion language of VST, leverages the formal soundness proof of VST, but allows users to describe functional correctness proofs intuitively by inserting assertions. VST-A analyzes control flow graphs, decomposes every C function into control flow paths between assertions, and reduces program verification problems into corresponding straightline Hoare triples. Compared to existing foundational program verification tools like VST and Iris, in VST-A, such decompositions and reductions are allowed to be nonstructural, which makes VST-A more flexible to use. VST-A's decomposition and reduction is defined in Coq, proved sound in Coq, and computed in a call-by-value way in Coq. The soundness proof for reduction is totally logical, independent of the complicated semantic model (and soundness proof) of VST's Hoare triple. Because of the rich assertion language, not all reduced proof goals can be automatically checked, but the system allows users to prove residual proof goals using the full power of the Coq proof assistant.

==> contents/not_used.tex <==

\subsection{Forward Symbolic Executor}
\label{sec:se}
Our work is based on a forward symbolic executor with two components:
    a symbolic assignment executor $\se(\cdot, \cdot)$
    and an assertion normalization program $\norm(\cdot)$.
We write $\findvalue{\Sigma; \Gamma}{\se(P, c)}{Q}$ if $Q$ is the result
    of symbolic execution,
i.e., given logical variable context $\Sigma$ and proposition context $\Gamma$,
    $\se(\cdot, \cdot)$ computes a strongest postcondition $Q$ for precondition $P$ and
    assignment statement $c$.
For example,
    in the reverse program given in \figref{fig:ll-reverse},
    if
    \begin{align*}
        \Sigma &:= a; b; l_1; l_2,\\
        \Gamma &:= \emptyset,\\
        P &:= \exists \ c \ x \ l_2'. \ l_2 = x \ l_2' \ \wedge \
            \denote{\cvar{w}}=a\ \wedge\ \denote{\cvar{v}}=b\ \wedge\ 
            b \mapsto (x, c) \ * \
            \ll\left(a, l_1\right) \ * \
            \ll\left(c, l_2'\right),\\
        c &:= \lstinline|t = v->tail|,
    \end{align*}
    then $\findvalue{\Sigma; \Gamma}{\se(P, c)}{Q}$ for
    \begin{align*}
        Q &:= \exists \ c \ x \ l_2'. \ l_2 = x \ l_2' \ \wedge \
            \denote{\cvar{w}}=a\ \wedge\ \denote{\cvar{v}}=b\ \wedge\ 
            \denote{\cvar{t}}=c\ \wedge\ 
            b \mapsto (x, c) \ * \
            \ll\left(a, l_1\right) \ * \
            \ll\left(c, l_2'\right).
    \end{align*}
Assignment executor may fail,
    if the precondition $P$ cannot guarantee $c$ can run successfully,
    or $P$ is not in a good form such that the symbolic executor can execute $c$.

Besides, an assertion normalization program turns an assertion into a \emph{better} form.
We write $\findvalue{\Sigma; \Gamma}{\norm(P)}{Q}$ if the $\norm(\cdot)$ program terminates
    and returns $Q$ when it tries to improve $P$.
Here, $P$ and $Q$ should be equivalent with each other but $Q$ is in a better form.
For example, the following assertion $I$ is the loop invariant in
    our reverse program (\figref{fig:ll-reverse}):
$$I:=\exists \ a \ b \ l_1 \ l_2. \ \denote{\cvar{w}} = a \ \wedge \
    \denote{\cvar{v}} = b \ \wedge \
    l = \rev(l_1) \ l_2 \ \wedge \
    \ll\left(a, l_1\right) \ * \
    \ll\left(b, l_2\right)$$
So at the beginning of the loop body, the assertion
    $(I\ \wedge\ \denote{\cvar{v}}=\btrue)$ must hold.
But this form may be not preferred by the symbolic executor and it becomes hard for next step.
Assertion normalization program handles this situation.
Here, $\findvalue{\Sigma; \Gamma}{\norm(I\land \denote{b}=\btrue)}{Q}$
for
$$Q:=\exists \ a \ b \ l_1 \ l_2. \ \denote{\cvar{w}} = a \ \wedge \
    \denote{\cvar{v}} = b \ \wedge \
    b\neq \cnull\ \wedge\ 
    l = \rev(l_1) \ l_2 \ \wedge \
    \ll\left(a, l_1\right) \ * \
    \ll\left(b, l_2\right).$$

VST provides an instance of forward symbolic executor inside.









\figref{fig:choarelogic} shows some proof rules of VST's Hoare logic.
Besides, \rulename{Exists} and \rulename{Pure} rules
    introduce variables and propositions from precondition to context, respectively.
\rulename{Loop}
    rule has two invariants, loop invariant $I$ and continue invariant $\coninv{I}$,
    that $I$ is the invariant must hold before each iteration,
    and $\coninv{I}$ is the invariant must hold at $\ccontinue$
    or before $\cincr{c}$ statement.
For return statements, we only demonstrate a proof rule for statements without a return value.
In our development, there is a similar proof rule with return value; we omit it here for simplicity.
\rulename{Assoc} rule reassociates sequential compositions\footnote{Although both directions of reassociation are sound, we only need one in this paper.}.

Different from ordinary versions, we demonstrate pre/postcondition replacement in an asymmetric way.
Specifically, \rulename{Pre} is our precondition strengthening rule.
But we do not have one corresponding rule for postcondition weakening.
Instead, it is built-in \rulename{Skip}, \rulename{Assignment},
    \rulename{Break}, \rulename{Continue} and \rulename{Return}.
We choose this special presentation because VST always suggests users
    verify programs in a forward direction.
For example, suppose $c$ is an assignment statement, using \rulename{Assignment},
   a triple with form $\hoareabbr{P}{c}{R}{R'}$
    can be reduced to an assertion entailment
    $\Sigma; \Gamma; Q \vDash R$ where $Q$ is the strongest postcondition
    generated by VST's assignment executor $\se(P, c)$.
As another example, $\hoareabbr{P}{(c; c_1); c_2}{R}{R'}$
    can be reduced
    $\hoareabbr{Q}{c_1; c_2}{R}{R'}$
    if $c$ is an assignment statement and $\findvalue{\Sigma; \Gamma}{\se(P, c)}{Q}$.
This reduction uses \rulename{Assoc}, \rulename{Seq}, \rulename{Assignment} and
    the reflexivity of assertion entailment.





Besides, VST also proves some other rules sound, including the reverse direction of \rulename{Assoc},
    normal postcondition weakening (\rulename{Post}).
Rule \rulename{IfSeq} and \rulename{NoContinue} are used for additional proof automation.
\begin{mathpar}
    \inferrule*[left=Post]{
        \Sigma; \Gamma; Q \entails R \and
        \hoareabbr{P}{c}{Q}{R'}
    } {
        \hoareabbr{P}{c}{R}{R'}
    }
    \and
    \inferrule*[left=IfSeq]{
        \hoareabbr{P}{(\cifthenelse{b}{c_1}{c_2}); c_3}{Q}{R}
    } {
        \hoareabbr{P}{\cifthenelse{b}{c_1;c_3}{c_2;c_3}}{Q}{R}
    }
    \and
    \inferrule*[left=NoContinue]{
        \Sigma; \Gamma; P \entails I \and
        \hoare{I}{c;\cincr{c}}{I}{Q}{\bot}{\retcnd{Q}}
    } {
        \hoare{P}{\cloop{c}{\cincr{c}}}{Q}{\brkcnd{Q}}{\concnd{Q}}{\retcnd{Q}}
    }
\end{mathpar}
Our development, VST-A, is built on the basis of those proof rules in \figref{fig:choarelogic}, \rulename{Post} and \rulename{NoContinue}.
All of these rules
    are proved sound foundationally in VST w.r.t. CompCert Clight semantics
    (if $\se(\cdot, \cdot)$ and $\norm(\cdot)$ are interpreted as VST's own assignment executor and normalization program).



==> contents/not_used_frontend.tex <==

\begin{figure}[tp]
    \centering
    \includegraphics[scale=0.15]{figures/Clightgen.png} %TODO update figure
    \caption{Front end structure}
    \label{fig:frontend}
\end{figure}

We have implemented a front end called ``Aclightgen'' for VST-A,
    which parses a commented C program and generates annotated program into 
    an abstract ClightA term in Coq.
The front-end program is implemented by applying minimal modifications on CompCert Clightgen,
    which generates Clight program that user wants to verify.
So this method allows us to easily guarantee the annotated program is 
    corresponding to original program.


\begin{figure}[h]
\begin{lstlisting}[language=C, mathescape=true, xleftmargin=2em,xrightmargin=1em, numbers=left, frame = {TB}]
struct list {unsigned head; struct list *tail;};
reverse_aclight := $\lambda \ l.   $
  $\Assert \  \ll\left(\denote{\cvar{p}}, l\right)$;
    w = NULL; v = p;
    $\textbf{loop}$ ($\cskip$) {
      if (v) { $\cskip$; } else { break; }
      $\ExGivensymbol \ l_1 \ c \ x \ l_2'.  $ {
          $\Assert \ \denote{\cvar{w}} = a \ \wedge \
              l = \rev(l_1) \ x \ l_2' \wedge \ 
              \denote{\cvar{v}} \mapsto (x, c) \ * \
              \ll\left(\denote{\cvar{w}}, l_1\right) \ * \
              \ll\left(c, l_2'\right)$;
          t = v->tail; v->tail = w; w = v; v = t;
      }
    }
    ret = w;
  $\Assert \ \ll\left(\denote{\cvar{ret}}, \rev(l)\right)$
\end{lstlisting}
    \caption{The ClightA definition that VST-A front end generates for \figref{fig:ll-reverse}}
    \label{fig:examplefrondend}
\end{figure}

\figref{fig:frontend} shows structure of VST-A's frontend comparing with
    CompCert's Clight generator (Clightgen).
\figref{fig:examplefrondend} shows an example result of parsing the assertion
    annotated linked-list reverse program in \figref{fig:ll-reverse}.
We present some key technial details for the VST-A front end below.


\begin{figure}[h]
\begin{subfigure}[b]{0.45\textwidth}
$$\begin{array}{rrl}
    \text{statement}:&c := &
    c_1; c_2\\
&\mid&  \cifthenelse{e}{c_1}{c_2}\\
&\mid&  \cloop{c_1}{c_2}\\
&\mid&  \cdots
\end{array}$$
\caption{Clight}
\end{subfigure}
~
\begin{subfigure}[b]{0.45\textwidth}
$$\begin{array}{rrl}
\text{statement}:&c := &
        \textsf|/*comment*/|\ c\\
&\mid&  c\ \textsf|/*comment*/|\\
&\mid&  c_1; c_2\\
&\mid&  \cifthenelse{e}{c_1}{c_2}\\
&\mid&  \cloop{c_1}{c_2}\\
&\mid&  \cdots
\end{array}$$
\caption{Clight with comment}
\end{subfigure}
    \caption{Syntax of Clight and Clight with comment}
    \label{fig:ClightC}
\end{figure}


\paragraph{Parsing and transformation}
Clightgen first parses C code and then does a series of transformations
    to Clight. %TODO
Our front end first includes comments as strings in parsing and syntax transformation.
We slightly modify Clightgen so that these comments are all preserved.
After parsing, Clightgen applies a series of transformations to convert C to Clight.
We modify the intermediate representations to preserve comments in this process.
\figref{fig:ClightC} shows the comparison between
    syntax of original Clight and our Clight-with-comment.
Two new syntactic combinators are added to represent comments on the left and right side of a statement.
We also apply similar changes to other intermediate representations
    and adapt each transformation step for preserving comments.
Our modifications are all local and small-scale.
Also, trivially eliminating comments can turn a Clight-with-comment program to the original Clight program.


\paragraph{Building annotations}
After getting program in Clight-with-comments,
    our front end analyzes the comments and build annotated programs with
    with annotations as OCaml strings.
To be specifc, the following steps are performed when building annotations.
\begin{itemize}
    \item \emph{Reassociating sequential compositions:}
    ClightA requests the left hand side of every sequential composition
        to be a single statement, so that
        each $\ExGivensymbol$ clause encloses all statements after it.
    Annotation building process puts statements in a sequential composition into a list,
        and fold them from right to left.
    \item \emph{Finding loop invariants:}
    Loop invariants are \emph{not compulsory} in VST-A annotated programs,
        as indicated by our linked list reverse example. Nevertheless, users are still able
        to specify them with \textsf{/* Inv ... */} in the comments. The annotation
        builder will insert them as assertions into correct positions in the ClightA term.
        % The transformations are proved to be sound in VST,
        % and VST also uses this transformation for such kind of loops.
    % Users can also \emph{provide no loop invariants}, as we will see in the 
        % next section, which does not need special treatment in parsing stage.
    \item \emph{Generating $\ExGivensymbol$ clauses: }
        VST suggests proving Hoare triples when precondition is in canonical 
        form without existential variables.
        Our VST-A framework shares the same idea by making existential variables explicit
            in the abstract syntax ClightA and split results.
        In order to parse an annotated C program, every assertion with existential variables
            will generate an $\ExGivensymbol$ clause in the target abstract syntax, 
            as shown in Line 7 of \figref{fig:examplefrondend}.
        Users do not need to write any $\ExGivensymbol$ clauses manually.
    \item \emph{Transforming function specifications: }
        We allow users to write function specification at the beginning of each function
            using $\With$, $\Require$ and $\Ensure$ keywords, as shown in Line 3-5 in \figref{fig:ll-reverse}. 
        This is an easy and clear way to write function specifications.
        Annotation builder extracts function specifications to the beginning
            and end of the function body.
        Assertions may also use variables mentioned in $\With$ clause.
        The whole ClightA program will be abstracted over $\With$ variables.
    
\end{itemize}


% \paragraph{Checking postconditions}
% As we show in Section~\ref{sec:revert},
%     annotation based verifier allows complex statements not followed by an assertion
%         if and only if the complex statement has only one normal exit point.
% If a complex statement is not followed by an assertion,
%     annotation builder checks whether it has only one normal exit point
%         using the algorithm shown in \figref{fig:countexit}.


\begin{figure}
\hspace*{-0.02\textwidth}
\begin{subfigure}[b]{0.5\textwidth}
$$\begin{array}{rrl}
    \text{string}:&s := & \cdots\\
    \text{statement}:&c := &
        \ExGivensymbol\ s_{x}\ s_{P}\ c\\
&\mid&  \Assert s\\
&\mid&  \cloop{c_1}{c_2}\\
&\mid&  \cdots
\end{array}$$
    \caption{Syntax of ClightA with string annotation}
\end{subfigure}
~
\begin{subfigure}[b]{0.5\textwidth}
$$\begin{array}{rrl}
    \text{assertion}:&P := & \cdots\\
    \text{identifier}:&x := & \cdots\\
    \text{type}:&A := & \cdots\\
    \text{statement}:&c := &
        \ExGiven{x}{A}{P(x)}{C} \\
&\mid&  \Assert P\\
&\mid&  \cloop{c_1}{c_2}\\
&\mid&  \cdots
\end{array}$$
    \caption{Syntax of ClightA with syntactic annotation}
\end{subfigure}
    \caption{Comparison between string annotation and syntactic annotation}
    \label{fig:compareprint}
\end{figure}
\paragraph{Printing}

And finally, our front end prints the annotated program
    to a Coq's ``.v'' file, where the annotated program is a formal Coq term.
It is worth mentioning that annotation builder generates ClightA with string annotation,
    instead of ClightA with syntactic annotation.
\figref{fig:compareprint} shows the differences between string annotation and syntactic annotation.
Strings are more flexible and easier to process.
When printing to Coq's ``.v'' file,
    string annotations are printed at proper positions
    and become syntactic annotation.

    


==> contents/not_used_split.tex <==

Similar to ClightA syntax $C_c$,
the split result is also parameterized by a simpler syntax in implementation.
For simple results, the assertion is treated simply as a placeholder and there are
no logical variables involved. For complete results, each result type is a Coq 
\textsf{Inductive} type with an extra constructor to introduce logical variables
into assertions. A complete result $p$ is of the dependepent type on a simple
result $p_s$ if $p$ and $p_s$ have identical basic statements.

We will show how this dependepent type based relation 
is useful in the split function
implementation in Coq in Section \ref{sec:split_fun}.






First, the $\restostm$ function converts sequences of basic program statements 
into the abstract C language. Note that the basic statements of split results no
longer contain control flow instructions such as $\cbreak$ and $\ccontinue$,
so for any $\restostm(\vec{c_{b}})$, we only care about the case when it 
exits with normal status. We assign a \textsf{True} assertion $\top$ to
post-condition fields other than normal. Besides, we make use of this
observation to interpret the conditional expression $e$. We simply encode it
into a simple if-branching structure that exit with $\cbreak$ if $e$ evaluates
to $\textsf{false}$. This encoding is safe since the break post-condition
is always $\top$, and the path in question only cares about the case
where $e$ evaluates to $\textsf{true}$.


For interpreting pre-partial paths, $\semaxpre$ takes a user-specified pre-condition $P$,
and interprets the result as a Hoare triple. This procedure is similar for $\semaxatom$,
the base case for $\semaxpost$, and the base case for  $\semaxpath$. 
For logical variables syntactically binded
to post-partial paths or full-paths, the interpretation function will convert them into
a Coq-level universal quantification.

% For return post-partial paths, since the post condition for return is
% parameterized by the return value. To match the VST program logic, we still make use
% of the $\creturn ?e$ statement and the returning post condition in VST during
% interpretation. Now we only care about the control flow that exits with return status,
% so other post-conditions are set as $\top$.

Finally, the $\semaxsplit$ function takes a split result and interprets it into
a conjunction of Hoare triples. All the interpretation functions are implemented
in Coq as functions that returns a proposition, which is left
for users as the verification goals towards program correctness.


\paragraph{Soundness of ex-given structure}
The premise that $$\semaxsplit(P_0,\vec{Q},\splitfun{(\ExGiven{x}{A}{P(x)}{c'})})$$
leads to the following two propositions.

\begin{enumerate}
    \item $P_0 \entails \EX{x}{A}{P(x)}$
    \item $\forall x:A. \ \semaxsplit(P(x), \vec{Q}, \splitfun{(c')})$
\end{enumerate}

The first proposition can be obtained from the head path 
$\singleton{ []\postassert{\EX{x}{A}{P(x)}} }$. The second proposition
can be obtained from the rest of the fields in the split result.
The soundness proof is done by first applying $\textsc{Semax-Conseq}$
to transform the pre-condition of the triple to be $\EX{x}{A}{P(x)}$.
Next, the $\textsc{Extract-Exists}$ rule is used to introduce the
existentially quantified $x$ into the proof context. Then the 
induction hypothesis and the second proposition above are applied
to complete the proof.

==> figures/c_hoare_primary.tex <==
% TODO: do we need to move typecheck premises into the precondition?
% Remark: omit the cast case since nothing special needs to be done
\begin{figure*}[h]
    \centering
    \begin{mathpar}
        \inferrule*[left=Semax-Set]{
            % \text{\textsf{x} is a nonaddressable variable} \and
            % \text{\textsf{x} and $e$ have compatible C scalar types} \and
            %  
            % {e} \hasvalue
        } {
             \hoareabbr{\later \left( {e} \hasvalue \land P[e/\textsf{x}]\right)}{\cassign{\textsf{x}}{e}}{P}{\bot}
        }
        \and
        \inferrule*[left=Semax-Load]{
            % \text{\textsf{x} is a nonaddressable variable} \and
            % \text{\textsf{x} and $e$ have compatible C scalar types} \and
            \pi \text{ is readable} 
            % \and
        } {
             \hoareabbr
                {\later  \left(\
                {\&e}\hasvalue{p} \land
                \left(p \mapsto_{\pi} v \sepcon \TT\right) \land P[v/\textsf{x}] \right)}
                {\cassign{\textsf{x}} {e}}
                {P}{\bot}
        }
        \and
        \inferrule*[left=Semax-Store]{
            % \text{$e_1$ and $e_2$ have compatible C scalar types} \and
            \pi \text{ is writable} \and
            % \findvalue{\Sigma; \Gamma} \and
            % \findvalue{\Sigma; \Gamma}
        } {
             \hoareabbr
                {\later \left(
                    {\&e_1}\hasvalue{p} \land
                    {e_2}\hasvalue{v'} \land
                p \mapsto_{\pi} v \sepcon \left( p \mapsto_{\pi} v' \wand P \right) \right)}
                { \cassign{e_1}{e_2}}
                {P}{\bot}
        }
        \and
        \inferrule*[left=Semax-Call]{
            \Delta(f) = \phi \and
            \text{$\phi$ is a precise specification} \\
            \phi \subsume \funspecabbr{\vec{x}:\vec{A}}{\lambda \vec{y}. P}{\lambda r. Q} \and
            % \findvalue{\Sigma; \Gamma}
        } {
             \hoareabbr
                { \later (
                    {\vec{e}}\hasvalue{\vec{b}} \land
                    \exists \vec{x}:\vec{A}.\  P \, \vec{b} \, \vec{x} \sepcon
                        \left( Q \, \textsf{a} \, \vec{x} \wand R \right) )}
                { \cassign{\textsf{a}}{f(\vec{e})}}
                {R}{\bot}
        }
    \end{mathpar}
    \caption[Proof rules of C Hoare logic (Part II: primary rules)]{Proof rules of C Hoare logic (Part II: primary rules)\footnotemark}
    \label{fig:choarelogic_primary}
\end{figure*}


==> figures/list_rev_aclight.tex <==
\begin{figure}[h]
\begin{lstlisting}[language=C, mathescape=true, xleftmargin=2em,xrightmargin=1em, numbers=left, frame = {TB}, escapechar=|]
reverse_aclight := $\lambda \ l.   $
  $\Assert \  \ll\left(\denote{\cvar{p}}, l\right)$;
  w = NULL; v = p;
  $\textbf{loop}$ ($\cskip$) {
    if (v) { $\cskip$; } else { break; }
    $\ExGivensymbol \ l_1 \ c \ x \ l_2'.  $ { |\label{code:aclightgen-exgiven} |
      $\Assert \ \denote{\cvar{w}} = a \ \wedge \
            l = \rev(l_1) \ x \ l_2' \wedge \ 
            \denote{\cvar{v}} \mapsto (x, c) \ * \
            \ll\left(\denote{\cvar{w}}, l_1\right) \ * \
            \ll\left(c, l_2'\right)$;
      t = v->tail; v->tail = w; w = v; v = t; } }
  ret = w;
  $\Assert \ \ll\left(\denote{\cvar{ret}}, \rev(l)\right)$
\end{lstlisting}
    \caption{The ClightA definition that VST-A front-end generates for \figref{fig:ll-reverse}}
    \label{fig:examplefrondend}
\end{figure}

